Optimal Installation for Electric Vehicle Wireless Charging Lanes

Range anxiety, the persistent worry about not having enough battery power to complete a trip, remains one of the major obstacles to widespread electric-vehicle adoption. As cities look to attract more users to adopt electric vehicles, the emergence of wireless in-motion car charging technology presents itself as a solution to range anxiety. For a limited budget, cities could face the decision problem of where to install these wireless charging units. With a heavy price tag, an installation without a careful study can lead to inefficient use of limited resources. In this work, we model the installation of wireless charging units as an integer programming problem. We use our basic formulation as a building block for different realistic scenarios, carry out experiments using real geospatial data, and compare our results to different heuristics.

==> mybbl.tex <==
\begin{thebibliography}{73}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Pan et~al.(2010)Pan, Bent, Berscheid, and
  Izraelevitz]{pan2010locating}
Feng Pan, Russell Bent, Alan Berscheid, and David Izraelevitz.
\newblock Locating phev exchange stations in v2g.
\newblock In \emph{Smart Grid Communications (SmartGridComm), 2010 First IEEE
  International Conference on}, pages 173--178. IEEE, 2010.

\bibitem[Vilathgamuwa and Sampath(2015)]{vilathgamuwa2015wireless}
DM~Vilathgamuwa and JPK Sampath.
\newblock Wireless power transfer for electric vehicles, present and future
  trends.
\newblock In \emph{Plug in electric vehicles in smart grids}, pages 33--60.
  Springer, 2015.

\bibitem[Li et~al.(2015)Li, Chowdhury, Bhavsar, and He]{li2015optimizing}
Z~Li, M~Chowdhury, P~Bhavsar, and Y~He.
\newblock Optimizing the performance of vehicle-to-grid (v2g) enabled battery
  electric vehicles through a smart charge scheduling model.
\newblock \emph{International Journal of Automotive Technology}, 16\penalty0
  (5):\penalty0 827--837, 2015.

\bibitem[Chen et~al.(2016)Chen, He, and Yin]{chen2016optimal}
Zhibin Chen, Fang He, and Yafeng Yin.
\newblock Optimal deployment of charging lanes for electric vehicles in
  transportation networks.
\newblock \emph{Transportation Research Part B: Methodological}, 91:\penalty0
  344--365, 2016.

\bibitem[He et~al.(2013{\natexlab{a}})He, Yin, and Zhou]{he2013integrated}
Fang He, Yafeng Yin, and Jing Zhou.
\newblock Integrated pricing of roads and electricity enabled by wireless power
  transfer.
\newblock \emph{Transportation Research Part C: Emerging Technologies},
  34:\penalty0 1--15, 2013{\natexlab{a}}.

\bibitem[Ko and Jang(2013)]{ko2013optimal}
Young~Dae Ko and Young~Jae Jang.
\newblock The optimal system design of the online electric vehicle utilizing
  wireless power transmission technology.
\newblock \emph{IEEE Transactions on Intelligent Transportation Systems},
  14\penalty0 (3):\penalty0 1255--1265, 2013.

\bibitem[Qiu et~al.(2013)Qiu, Chau, Liu, and Chan]{qiu2013overview}
Chun Qiu, KT~Chau, Chunhua Liu, and CC~Chan.
\newblock Overview of wireless power transfer for electric vehicle charging.
\newblock In \emph{Electric Vehicle Symposium and Exhibition (EVS27), 2013
  World}, pages 1--9. IEEE, 2013.

\bibitem[Bi et~al.(2016)Bi, Kan, Mi, Zhang, Zhao, and Keoleian]{bi2016review}
Zicheng Bi, Tianze Kan, Chunting~Chris Mi, Yiming Zhang, Zhengming Zhao, and
  Gregory~A Keoleian.
\newblock A review of wireless power transfer for electric vehicles: Prospects
  to enhance sustainable mobility.
\newblock \emph{Applied Energy}, 179:\penalty0 413--425, 2016.

\bibitem[Li and Mi(2015)]{li2015wireless}
Siqi Li and Chunting~Chris Mi.
\newblock Wireless power transfer for electric vehicle applications.
\newblock \emph{IEEE journal of emerging and selected topics in power
  electronics}, 3\penalty0 (1):\penalty0 4--17, 2015.

\bibitem[Lukic and Pantic(2013)]{lukic2013cutting}
Srdjan Lukic and Zeljko Pantic.
\newblock Cutting the cord: Static and dynamic inductive wireless charging of
  electric vehicles.
\newblock \emph{IEEE Electrification Magazine}, 1\penalty0 (1):\penalty0
  57--64, 2013.

\bibitem[Cirimele et~al.(2014)Cirimele, Freschi, and
  Guglielmi]{cirimele2014wireless}
Vincenzo Cirimele, Fabio Freschi, and Paolo Guglielmi.
\newblock Wireless power transfer structure design for electric vehicle in
  charge while driving.
\newblock In \emph{Electrical Machines (ICEM), 2014 International Conference
  on}, pages 2461--2467. IEEE, 2014.

\bibitem[Fuller(2016)]{fuller2016wireless}
Micah Fuller.
\newblock Wireless charging in california: Range, recharge, and vehicle
  electrification.
\newblock \emph{Transportation Research Part C: Emerging Technologies},
  67:\penalty0 343--356, 2016.

\bibitem[Ning et~al.(2013)Ning, Miller, Onar, and White]{ning2013compact}
Puqi Ning, John~M Miller, Omer~C Onar, and Clifford~P White.
\newblock A compact wireless charging system for electric vehicles.
\newblock In \emph{Energy Conversion Congress and Exposition (ECCE), 2013
  IEEE}, pages 3629--3634. IEEE, 2013.

\bibitem[Cho and Kim(2011)]{cho2011magnetic}
DH~Cho and J~Kim.
\newblock Magnetic field design for low emf and high efficiency wireless power
  transfer system in on-line electric vehicle.
\newblock In \emph{CIRP Design Conference 2011}, 2011.

\bibitem[Lee et~al.(2010)Lee, Huh, Park, Choi, Cho, and Rim]{lee2010line}
Sungwoo Lee, Jin Huh, Changbyung Park, Nam-Sup Choi, Gyu-Hyeoung Cho, and
  Chun-Taek Rim.
\newblock On-line electric vehicle using inductive power transfer system.
\newblock In \emph{2010 IEEE Energy Conversion Congress and Exposition}, pages
  1598--1601. IEEE, 2010.

\bibitem[Kim et~al.(2012)Kim, Son, Shin, Shin, Song, Lee, Jung, and
  Jeon]{kim2012design}
Yangsu Kim, Youngdong Son, Seungyong Shin, Jaegue Shin, Boyune Song, Seokhwan
  Lee, Guho Jung, and Seongjeub Jeon.
\newblock Design of a regulator for multi-pick-up systems through using current
  offsets.
\newblock In \emph{Electric Vehicle Conference (IEVC), 2012 IEEE
  International}, pages 1--6. IEEE, 2012.

\bibitem[Jung et~al.(2012)Jung, Song, Shin, Lee, Shin, Kim, and
  Jeon]{jung2012high}
Guho Jung, Boyune Song, Seungyong Shin, Seokhwan Lee, Jaegue Shin, Yangsu Kim,
  and Sungjeub Jeon.
\newblock High efficient inductive power supply and pickup system for on-line
  electric bus.
\newblock In \emph{Electric Vehicle Conference (IEVC), 2012 IEEE
  International}, pages 1--5. IEEE, 2012.

\bibitem[Gill et~al.(2014)Gill, Bhavsar, Chowdhury, Johnson, Taiber, and
  Fries]{gill2014infrastructure}
Jasprit~S Gill, Parth Bhavsar, Mashrur Chowdhury, Jennifer Johnson, Joachim
  Taiber, and Ryan Fries.
\newblock Infrastructure cost issues related to inductively coupled power
  transfer for electric vehicles.
\newblock \emph{Procedia Computer Science}, 32:\penalty0 545--552, 2014.

\bibitem[Mohrehkesh and Nadeem(2011)]{mohrehkesh2011toward}
Shahram Mohrehkesh and Tamer Nadeem.
\newblock Toward a wireless charging for battery electric vehicles at traffic
  intersections.
\newblock In \emph{2011 14th International IEEE Conference on Intelligent
  Transportation Systems (ITSC)}, pages 113--118. IEEE, 2011.

\bibitem[Sarker et~al.(2016)Sarker, Qiu, Shen, Gil, Taiber, Chowdhury, Martin,
  Devine, and Rindos]{sarker2016efficient}
Ankur Sarker, Chenxi Qiu, Haiying Shen, Andrea Gil, Joachim Taiber, Mashrur
  Chowdhury, Jim Martin, Mac Devine, and AJ~Rindos.
\newblock An efficient wireless power transfer system to balance the state of
  charge of electric vehicles.
\newblock In \emph{Parallel Processing (ICPP), 2016 45th International
  Conference on}, pages 324--333. IEEE, 2016.

\bibitem[Johnson et~al.(2013)Johnson, Chowdhury, He, and
  Taiber]{johnson2013utilizing}
Jennifer Johnson, Mashrur Chowdhury, Yiming He, and Joachim Taiber.
\newblock Utilizing real-time information transferring potentials to vehicles
  to improve the fast-charging process in electric vehicles.
\newblock \emph{Transportation Research Part C: Emerging Technologies},
  26:\penalty0 352--366, 2013.

\bibitem[Li et~al.(2016)Li, Dey, Chowdhury, and Bhavsar]{li2016connectivity}
Zhiyun Li, Kakan Dey, Mashrur Chowdhury, and Parth Bhavsar.
\newblock Connectivity supported dynamic routing of electric vehicles in an
  inductively coupled power transfer environment.
\newblock \emph{IET Intelligent Transport Systems}, 2016.

\bibitem[He et~al.(2013{\natexlab{b}})He, Wu, Yin, and Guan]{he2013optimal}
Fang He, Di~Wu, Yafeng Yin, and Yongpei Guan.
\newblock Optimal deployment of public charging stations for plug-in hybrid
  electric vehicles.
\newblock \emph{Transportation Research Part B: Methodological}, 47:\penalty0
  87--101, 2013{\natexlab{b}}.

\bibitem[Kang and Recker(2014)]{kang2014strategic}
Jee~Eun Kang and Will Recker.
\newblock Strategic hydrogen refueling station locations with scheduling and
  routing considerations of individual vehicles.
\newblock \emph{Transportation Science}, 49\penalty0 (4):\penalty0 767--783,
  2014.

\bibitem[Jung et~al.(2014)Jung, Chow, Jayakrishnan, and
  Park]{jung2014stochastic}
Jaeyoung Jung, Joseph~YJ Chow, R~Jayakrishnan, and Ji~Young Park.
\newblock Stochastic dynamic itinerary interception refueling location problem
  with queue delay for electric taxi charging stations.
\newblock \emph{Transportation Research Part C: Emerging Technologies},
  40:\penalty0 123--142, 2014.

\bibitem[He et~al.(2015)He, Yin, and Zhou]{he2015deploying}
Fang He, Yafeng Yin, and Jing Zhou.
\newblock Deploying public charging stations for electric vehicles on urban
  road networks.
\newblock \emph{Transportation Research Part C: Emerging Technologies},
  60:\penalty0 227--240, 2015.

\bibitem[Jang et~al.(2012{\natexlab{a}})Jang, Ko, and Jeong]{jang2012optimal}
Young~Jae Jang, Young~Dae Ko, and Seungmin Jeong.
\newblock Optimal design of the wireless charging electric vehicle.
\newblock In \emph{Electric Vehicle Conference (IEVC), 2012 IEEE
  International}, pages 1--5. IEEE, 2012{\natexlab{a}}.

\bibitem[Jang et~al.(2012{\natexlab{b}})Jang, Ko, and Jeong]{jang2012creating}
Young~Jae Jang, Young~Dae Ko, and Seungmin Jeong.
\newblock Creating innovation with systems integration, road and vehicle
  integrated electric transportation system.
\newblock In \emph{Systems Conference (SysCon), 2012 IEEE International}, pages
  1--4. IEEE, 2012{\natexlab{b}}.

\bibitem[Mouhrim et~al.(2016)Mouhrim, Alaoui, and
  Boukachour]{mouhrim2016optimal}
Nisrine Mouhrim, Ahmed El~Hilali Alaoui, and Jaouad Boukachour.
\newblock Optimal allocation of wireless power transfer system for electric
  vehicles in a multipath environment.
\newblock In \emph{Logistics Operations Management (GOL), 2016 3rd
  International Conference on}, pages 1--7. IEEE, 2016.

\bibitem[Church and Velle(1974)]{church1974maximal}
Richard Church and Charles~R Velle.
\newblock The maximal covering location problem.
\newblock \emph{Papers in regional science}, 32\penalty0 (1):\penalty0
  101--118, 1974.

\bibitem[Farahani et~al.(2012)Farahani, Asgari, Heidari, Hosseininia, and
  Goh]{farahani2012covering}
Reza~Zanjirani Farahani, Nasrin Asgari, Nooshin Heidari, Mahtab Hosseininia,
  and Mark Goh.
\newblock Covering problems in facility location: A review.
\newblock \emph{Computers \& Industrial Engineering}, 62\penalty0 (1):\penalty0
  368--407, 2012.

\bibitem[Daskin(2008)]{daskin2008you}
Mark~S Daskin.
\newblock What you should know about location modeling.
\newblock \emph{Naval Research Logistics (NRL)}, 55\penalty0 (4):\penalty0
  283--294, 2008.

\bibitem[Hale and Moberg(2003)]{hale2003location}
Trevor~S Hale and Christopher~R Moberg.
\newblock Location science research: a review.
\newblock \emph{Annals of operations research}, 123\penalty0 (1):\penalty0
  21--35, 2003.

\bibitem[Hodgson(1990)]{hodgson1990flow}
M~John Hodgson.
\newblock A flow-capturing location-allocation model.
\newblock \emph{Geographical Analysis}, 22\penalty0 (3):\penalty0 270--279,
  1990.

\bibitem[Kuby and Lim(2005)]{kuby2005flow}
Michael Kuby and Seow Lim.
\newblock The flow-refueling location problem for alternative-fuel vehicles.
\newblock \emph{Socio-Economic Planning Sciences}, 39\penalty0 (2):\penalty0
  125--145, 2005.

\bibitem[Kuby and Lim(2007)]{kuby2007location}
Michael Kuby and Seow Lim.
\newblock Location of alternative-fuel stations using the flow-refueling
  location model and dispersion of candidate sites on arcs.
\newblock \emph{Networks and Spatial Economics}, 7\penalty0 (2):\penalty0
  129--152, 2007.

\bibitem[Upchurch et~al.(2009)Upchurch, Kuby, and Lim]{upchurch2009model}
Christopher Upchurch, Michael Kuby, and Seow Lim.
\newblock A model for location of capacitated alternative-fuel stations.
\newblock \emph{Geographical Analysis}, 41\penalty0 (1):\penalty0 85--106,
  2009.

\bibitem[Kim and Kuby(2012)]{kim2012deviation}
Jong-Geun Kim and Michael Kuby.
\newblock The deviation-flow refueling location model for optimizing a network
  of refueling stations.
\newblock \emph{international journal of hydrogen energy}, 37\penalty0
  (6):\penalty0 5406--5420, 2012.

\bibitem[Huang et~al.(2015)Huang, Li, and Qian]{huang2015optimal}
Yongxi Huang, Shengyin Li, and Zhen~Sean Qian.
\newblock Optimal deployment of alternative fueling stations on transportation
  networks considering deviation paths.
\newblock \emph{Networks and Spatial Economics}, 15\penalty0 (1):\penalty0
  183--204, 2015.

\bibitem[Kim and Kuby(2013)]{kim2013network}
Jong-Geun Kim and Michael Kuby.
\newblock A network transformation heuristic approach for the deviation flow
  refueling location model.
\newblock \emph{Computers \& Operations Research}, 40\penalty0 (4):\penalty0
  1122--1131, 2013.

\bibitem[Wang and Lin(2013)]{wang2013locating}
Ying-Wei Wang and Chuah-Chih Lin.
\newblock Locating multiple types of recharging stations for battery-powered
  electric vehicle transport.
\newblock \emph{Transportation Research Part E: Logistics and Transportation
  Review}, 58:\penalty0 76--87, 2013.

\bibitem[Riemann et~al.(2015)Riemann, Wang, and Busch]{riemann2015optimal}
Raffaela Riemann, David~ZW Wang, and Fritz Busch.
\newblock Optimal location of wireless charging facilities for electric
  vehicles: flow-capturing location model with stochastic user equilibrium.
\newblock \emph{Transportation Research Part C: Emerging Technologies},
  58:\penalty0 1--12, 2015.

\bibitem[Wang and Lin(2009)]{wang2009locating}
Ying-Wei Wang and Chuah-Chih Lin.
\newblock Locating road-vehicle refueling stations.
\newblock \emph{Transportation Research Part E: Logistics and Transportation
  Review}, 45\penalty0 (5):\penalty0 821--829, 2009.

\bibitem[Wang and Wang(2010)]{wang2010locating}
Ying-Wei Wang and Chuan-Ren Wang.
\newblock Locating passenger vehicle refueling stations.
\newblock \emph{Transportation Research Part E: Logistics and Transportation
  Review}, 46\penalty0 (5):\penalty0 791--801, 2010.

\bibitem[Wang(2011)]{wang2011locating}
Ying-Wei Wang.
\newblock Locating flow-recharging stations at tourist destinations to serve
  recreational travelers.
\newblock \emph{International Journal of Sustainable Transportation},
  5\penalty0 (3):\penalty0 153--171, 2011.

\bibitem[Dong et~al.(2014)Dong, Liu, and Lin]{dong2014charging}
Jing Dong, Changzheng Liu, and Zhenhong Lin.
\newblock Charging infrastructure planning for promoting battery electric
  vehicles: An activity-based approach using multiday travel data.
\newblock \emph{Transportation Research Part C: Emerging Technologies},
  38:\penalty0 44--55, 2014.

\bibitem[Bogaert et~al.(2005)Bogaert, Fack, Van~de Weghe, and
  De~Maeyer]{bogaert2005line}
Peter Bogaert, Veerle Fack, Nico Van~de Weghe, and Philippe De~Maeyer.
\newblock On line graphs and road networks.
\newblock In \emph{topology and Spatial Databases Workshop, Glasgow, Scotland},
  2005.

\bibitem[Winter(2002)]{Winter2002}
Stephan Winter.
\newblock Modeling costs of turns in route planning.
\newblock \emph{GeoInformatica}, 6\penalty0 (4):\penalty0 345--361, Dec 2002.
\newblock ISSN 1573-7624.
\newblock \doi{10.1023/A:1020853410145}.
\newblock URL \url{https://doi.org/10.1023/A:1020853410145}.

\bibitem[Chang(2013)]{chang2013state}
Wen-Yeau Chang.
\newblock The state of charge estimating methods for battery: A review.
\newblock \emph{ISRN Applied Mathematics}, 2013, 2013.

\bibitem[Wang et~al.(2016)Wang, Wang, Wang, Li, Ahmed, Habibi, and
  Emadi]{wang2016comparison}
Weizhong Wang, Deqiang Wang, Xiao Wang, Tongrui Li, Ryan Ahmed, Saeid Habibi,
  and Ali Emadi.
\newblock Comparison of kalman filter-based state of charge estimation
  strategies for li-ion batteries.
\newblock In \emph{Transportation Electrification Conference and Expo (ITEC),
  2016 IEEE}, pages 1--6. IEEE, 2016.

\bibitem[Koirala et~al.(2015)Koirala, He, and Shen]{koirala2015comparison}
Narayani Koirala, Fengxian He, and Weixiang Shen.
\newblock Comparison of two battery equivalent circuit models for state of
  charge estimation in electric vehicles.
\newblock In \emph{Industrial Electronics and Applications (ICIEA), 2015 IEEE
  10th Conference on}, pages 17--22. IEEE, 2015.

\bibitem[US(2017)]{fuelecon}
US.
\newblock Fuel economy.
\newblock \url{http://fueleconomy.gov/}, 2017.
\newblock Accessed: 03-29-2017.

\bibitem[Wu et~al.(2015)Wu, Freese, Cabrera, and Kitch]{wu2015electric}
Xinkai Wu, David Freese, Alfredo Cabrera, and William~A Kitch.
\newblock Electric vehicles’ energy consumption measurement and estimation.
\newblock \emph{Transportation Research Part D: Transport and Environment},
  34:\penalty0 52--67, 2015.

\bibitem[Fontana(2013)]{fontana2013optimal}
Matthew~William Fontana.
\newblock \emph{Optimal routes for electric vehicles facing uncertainty,
  congestion, and energy constraints}.
\newblock PhD thesis, Massachusetts Institute of Technology, 2013.

\bibitem[Watrin et~al.(2012)Watrin, Blunier, and Miraoui]{watrin2012review}
Nicolas Watrin, Benjamin Blunier, and Abdellatif Miraoui.
\newblock Review of adaptive systems for lithium batteries state-of-charge and
  state-of-health estimation.
\newblock In \emph{Transportation Electrification Conference and Expo (ITEC),
  2012 IEEE}, pages 1--6. IEEE, 2012.

\bibitem[Zhang et~al.(2015)Zhang, Li, Pei, and Zhu]{zhang2015integrated}
Cheng Zhang, Kang Li, Lei Pei, and Chunbo Zhu.
\newblock An integrated approach for real-time model-based state-of-charge
  estimation of lithium-ion batteries.
\newblock \emph{Journal of Power Sources}, 283:\penalty0 24--36, 2015.

\bibitem[Sun et~al.(2016)Sun, Xiong, and He]{sun2016systematic}
Fengchun Sun, Rui Xiong, and Hongwen He.
\newblock A systematic state-of-charge estimation framework for multi-cell
  battery pack in electric vehicles using bias correction technique.
\newblock \emph{Applied Energy}, 162:\penalty0 1399--1409, 2016.

\bibitem[Greenleaf et~al.(2015)Greenleaf, Dalchand, Li, and
  Zheng]{greenleaf2015temperature}
Michael Greenleaf, Omesh Dalchand, Hui Li, and Jim~P Zheng.
\newblock A temperature-dependent study of sealed lead-acid batteries using
  physical equivalent circuit modeling with impedance spectra derived high
  current/power correction.
\newblock \emph{IEEE Transactions on Sustainable Energy}, 6\penalty0
  (2):\penalty0 380--387, 2015.

\bibitem[Stetzel et~al.(2015)Stetzel, Aldrich, Trimboli, and
  Plett]{stetzel2015electrochemical}
Kirk~D Stetzel, Lukas~L Aldrich, M~Scott Trimboli, and Gregory~L Plett.
\newblock Electrochemical state and internal variables estimation using a
  reduced-order physics-based model of a lithium-ion cell and an extended
  kalman filter.
\newblock \emph{Journal of Power Sources}, 278:\penalty0 490--505, 2015.

\bibitem[Franke et~al.(2012)Franke, Neumann, B{\"u}hler, Cocron, and
  Krems]{franke2012experiencing}
Thomas Franke, Isabel Neumann, Franziska B{\"u}hler, Peter Cocron, and Josef~F
  Krems.
\newblock Experiencing range in an electric vehicle: Understanding
  psychological barriers.
\newblock \emph{Applied Psychology}, 61\penalty0 (3):\penalty0 368--391, 2012.

\bibitem[Newman(2010)]{Newman:2010:NI}
Mark Newman.
\newblock \emph{Networks: An Introduction}.
\newblock Oxford University Press, Inc., New York, NY, USA, 2010.
\newblock ISBN 0199206651, 9780199206650.

\bibitem[Freeman(1978)]{freeman1978centrality}
Linton~C Freeman.
\newblock Centrality in social networks conceptual clarification.
\newblock \emph{Social networks}, 1\penalty0 (3):\penalty0 215--239, 1978.

\bibitem[Borgatti(1995)]{borgatti1995centrality}
Stephen~P Borgatti.
\newblock Centrality and aids.
\newblock \emph{Connections}, 18\penalty0 (1):\penalty0 112--114, 1995.

\bibitem[Newman(2008)]{newman2008mathematics}
Mark~EJ Newman.
\newblock The mathematics of networks.
\newblock \emph{The new palgrave encyclopedia of economics}, 2\penalty0
  (2008):\penalty0 1--12, 2008.

\bibitem[Hart et~al.(2011)Hart, Watson, and Woodruff]{hart2011pyomo}
William~E Hart, Jean-Paul Watson, and David~L Woodruff.
\newblock Pyomo: modeling and solving mathematical programs in python.
\newblock \emph{Mathematical Programming Computation}, 3\penalty0 (3):\penalty0
  219--260, 2011.

\bibitem[Hart et~al.(2012)Hart, Laird, Watson, and Woodruff]{hart2012pyomo}
William~E Hart, Carl Laird, Jean-Paul Watson, and David~L Woodruff.
\newblock \emph{Pyomo--optimization modeling in python}, volume~67.
\newblock Springer Science \& Business Media, 2012.

\bibitem[ILOG(2014)]{ilog2014cplex}
IBM ILOG.
\newblock Cplex optimization studio.
\newblock
  \url{http://www-01.ibm.com/software/commerce/optimization/cplex-optimizer},
  2014.

\bibitem[Leskovec et~al.(2009)Leskovec, Lang, Dasgupta, and
  Mahoney]{leskovec2009community}
Jure Leskovec, Kevin~J Lang, Anirban Dasgupta, and Michael~W Mahoney.
\newblock Community structure in large networks: Natural cluster sizes and the
  absence of large well-defined clusters.
\newblock \emph{Internet Mathematics}, 6\penalty0 (1):\penalty0 29--123, 2009.

\bibitem[Haklay and Weber(2008)]{haklay2008openstreetmap}
Mordechai Haklay and Patrick Weber.
\newblock Openstreetmap: User-generated street maps.
\newblock \emph{IEEE Pervasive Computing}, 7\penalty0 (4):\penalty0 12--18,
  2008.

\bibitem[Bar-Gera(2009)]{bar2009transportation}
Hillel Bar-Gera.
\newblock Transportation test problems.
\newblock \emph{Website: http://www. bgu. ac. il/\~{} bargera/tntp/. Accessed
  April}, 28:\penalty0 2009, 2009.

\bibitem[Khan et~al.(2017)Khan, Chowdhury, Khan, Safro, and
  Ushijima-Mwesigwa]{khan2017utility}
MD~Khan, Mashrur Chowdhury, Sakib~Mahmud Khan, Ilya Safro, and Hayato
  Ushijima-Mwesigwa.
\newblock Utility maximization framework for opportunistic wireless electric
  vehicle charging.
%\newblock \emph{arXiv preprint arXiv:1708.07526}, 2017.
\newblock \emph{Transportation Research Board 97th Annual Meeting, Transportation Research Board,} 2018

\bibitem[Gutfraind et~al.(2015)Gutfraind, Safro, and
  Meyers]{gutfraind2015multiscale}
Alexander Gutfraind, Ilya Safro, and Lauren~Ancel Meyers.
\newblock Multiscale network generation.
\newblock In \emph{Information Fusion (Fusion), 2015 18th International
  Conference on}, pages 158--165. IEEE, 2015.

\bibitem[Staudt et~al.(2016)Staudt, Hamann, Safro, Gutfraind, and
  Meyerhenke]{staudt2016generating}
Christian~L Staudt, Michael Hamann, Ilya Safro, Alexander Gutfraind, and
  Henning Meyerhenke.
\newblock Generating scaled replicas of real-world complex networks.
\newblock In \emph{International Workshop on Complex Networks and their
  Applications}, pages 17--28. Springer, 2016.

\end{thebibliography}
